AugSumm: towards generalizable speech summarization using synthetic labels from large language model

Abstractive speech summarization (SSUM) aims to generate human-like summaries from speech. Given variations in information captured and phrasing, recordings can be summarized in multiple ways. Therefore, it is more reasonable to consider a probabilistic distribution of all potential summaries rather than a single summary. However, conventional SSUM models are mostly trained and evaluated with a single ground-truth (GT) human-annotated deterministic summary for every recording. Generating multiple human references would be ideal to better represent the distribution statistically, but is impractical because annotation is expensive. We tackle this challenge by proposing AugSumm, a method to leverage large language models (LLMs) as a proxy for human annotators to generate augmented summaries for training and evaluation. First, we explore prompting strategies to generate synthetic summaries from ChatGPT. We validate the quality of synthetic summaries using multiple metrics including human evaluation, where we find that summaries generated using AugSumm are perceived as more valid to humans. Second, we develop methods to utilize synthetic summaries in training and evaluation. Experiments on How2 demonstrate that pre-training on synthetic summaries and fine-tuning on GT summaries improves ROUGE-L by 1 point on both GT and AugSumm-based test sets. AugSumm summaries are available at https://github.com/Jungjee/AugSumm.

==> figs/prompt_DS_word.tex <==
\begin{figure}[ht]
\centering
\noindent\fbox{%
\parbox{0.95\linewidth }{%
    \footnotesize 
    \textit{You are here to create an extractive summary from the transcript. An extractive summary uses words from the input to convey the important portions of the video. Please make sure that the summary has between 40 and 60 words. Respond with only the extractive summary for: $\{$transcription$\}$.}
    
    \textit{transcription:} 
    
}}
\caption{Prompt for extractive AugSumm in word-level, directly generated using the transcript only without GT summary.}
\label{fig:prompt_DS_word}
\end{figure}
